Optimal Self-Stabilizing Mobile Byzantine-Tolerant Regular Register with bounded timestamp

This paper proposes the first implementation of a self-stabilizing regular register emulated by $n$ servers that is tolerant to both mobile Byzantine agents, and \emph{transient failures} in a round-free synchronous model. Differently from existing Mobile Byzantine tolerant register implementations, this paper considers a more powerful adversary where (i) the message delay (i.e., $\delta$) and the period of mobile Byzantine agents movement (i.e., $\Delta$) are completely decoupled and (ii) servers are not aware of their state i.e., they do not know if they have been corrupted or not by a mobile Byzantine agent.The proposed protocol tolerates \emph{(i)} any number of transient failures, and \emph{(ii)} up to $f$ Mobile Byzantine agents. In addition, our implementation uses bounded timestamps from the $\mathcal{Z}\_{13}$ domain and it is optimal with respect to the number of servers needed to tolerate $f$ mobile Byzantine agents in the given model.

==> cum.tex <==
% !TEX root = main.tex

In \cite{BDPT16c}, Bonomi \emph{et al.} proved that having a ${\sf maintenance}()$ operation, i.e., an operation that allows cured servers to restore a valid state and avoid the loss of the register value, is a necessary condition to implement a safe register in presence of MBF.

The ${\sf maintenance}()$ operation is specified as follow:

\begin{definition}[${\sf maintenance}()$ and $\mathcal{A}_{M}$]
A ${\sf maintenance}()$ operation is an operation that, when executed by a process $p_i$, terminates at some time $t$ leaving $p_i$ with a valid state at time $t$  (i.e., it guarantees that $p_i$ is correct at time $t$).
A maintenance algorithm $\mathcal{A}_{M}$ is an algorithm that implements the ${\sf maintenance}()$ operation.	
\end{definition}

This result naturally applies when considering also transient failures from which the following Corollary follows:

\begin{corollary}\label{th:maintenanceNecessity}
Let $n$ be the number of servers emulating a safe register and let $f$ be the number of Mobile Byzantine Agents affecting servers.
Let $\mathcal{A}_{R}$ and $\mathcal{A}_{W}$ be respectively the algorithms implementing the ${\sf read}()$ and the ${\sf write}()$ operation assuming no communication between servers.
If $f>0$ then there exists no protocol $\mathcal{P}_{reg}=\{\mathcal{A}_{R}, \mathcal{A}_{W}\}$ implementing a self-stabilising safe register in any of the MBF models for round-free computations.
\end{corollary}



Another necessary condition for the implementation of a register in the $(\Delta S, CUM)$ MBF model is the definition of a unique ${\sf maintenance}()$ operation that should be executed by both correct and cured servers. In $(*, CUM)$ models, in fact, even in the absence of transient failures, servers are not aware about their local state correctness (due to the fact that they cannot know if they are correct, cured or faulty). 
Thus, they cannot run different algorithms when they are correct or cured (or take different steps according to their failure state as in $(*, CAM)$ models). 
So, the ${\sf maintenance}()$ operation must be able to work \vir{not trusting} information stored locally but rather inferring the correct state from the information provided by other servers. %What we know is that the information servers are storing at the beginning of the \op{maintenance} operation may be not correct, but there is a fraction of correct servers storing correct information. Thus what we can do is to exchange those information to get the correct state and overwrite the current state. 

%
%\SB{Check again from here}
%
%
%%In the following we will prove other necessary conditions that any self-stabilising protocol $\mathcal{P}_{reg}$ must satisfy in order to provide a correct emulation of a regular register in the $(\Delta S, CUM)$ model.
%
%
%% Teorema Bonomi Del Pozzo
%
%\begin{theorem}\label{th:maintenanceNoInternalInput}
%Let $\mathcal{A}_M$ be a deterministic algorithm run by $s_i$ to implement the \op{maintenance} operation. Let $I_{ext}$ and $I_{int}$ be the algorithm external and internal input respectively, i.e., input deriving from the interaction between $p_i$ and other servers and input deriving from the $s_i$ internal state. There not exists $\mathcal{A}_M(I_{ext},I_{int})$ for the $(*, CUM)$ model.  
%\end{theorem}
%
%
%
%\begin{definition}[Safe Window $w_i$]
%A safe window $w_i$ is the temporal window $[T_i, T_{i+1}]$.
%\end{definition}
%
%
%
%\begin{corollary}\label{c:maintenanceInput}
%From Theorem \ref{th:maintenanceNoInternalInput} it follows that in the $(*, CUM)$ models, each algorithm $\mathcal{A}_M$ has as input only information coming from the interaction with the external environment during a safe window.
%\end{corollary}
%


==> detailedDescr.tex <==

\noindent{\bf Local variables at client $c_i$.} Each client $c_i$ maintains two sets $reply_i$ that is used during the ${\sf read}()$ operation to collect the three tuples $\langle j, \langle v, sn \rangle \rangle$ sent back from servers. 
Additionally, if $c_i$ is the writer, it maintains a local sequence number $csn$ that is incremented, respect to the $\mathcal{Z}_{13}$ arithmetic, each time it invokes a ${\sf write}()$ operation, which is timestamped with such sequence number.\\

\noindent{\bf Local variables at server $s_i$.} Each server $s_i$ maintains the following local variables: 
\begin{itemize}

	%\item {$V_i[0..2]$}: an array such that $V_i[0]=\ang{val_0}{sn_0}$, $V_i[1]=\ang{val_1}{sn_1}$ and $V_i[2]=\ang{val_2}{sn_2}$ such that $sn_2 -_6 sn_1 \leq 2$ and $sn_1 -_6 sn_0 \leq 1$ and $sn_k \in \mathcal{Z}_6, k \in \{0,1,2\}$. This array, when a server is correct is expected to be completely filled with three values. This set is reset and repopulated at each \op{maintenance} operation.
	
%\noindent{\bf -} 

\item $V_i$: a set containing $3$ tuples $\langle v, sn \rangle$, where $v$ is a value and $sn$ the corresponding sequence number.
%\noindent{\bf -} 
\item$V_{safe_i}$: this set has the same characteristic as $V_i$, and is populated by the function ${\sf insert}(V_{safe_i}, \langle v_k, sn_k \rangle)$.%\\ % places the new value in $V_{safe_i}$ according to the incremental order and if dimensions exceed $3$ then it discards from $V_{safe_i}$ the value associated to the lowest $sn$.
%\noindent{\bf -} 
\item $W_i$: a set where $s_i$ stores values coming directly from the writer, associating to it a timer, $\langle v, sn, timer \rangle$. When the timer expires, the associated value is deleted.
%\noindent{\bf -} 
\item $echo\_vals_i$ and $echo\_read_i$: two sets used to collect information propagated through {\sc echo} messages. The first one stores tuple $\langle v, sn \rangle_j $. The set $echo\_read_i$ contains identifiers of concurrently reading clients in order to notify cured servers and expedite termination of ${\sf read}()$.
%\noindent{\bf -} 
\item$pending\_read_i$: set variable used to collect identifiers of the clients that are currently reading. Notice, for simplicity we do not explicitly manage the values discharge from such set since it has no impact on the protocol correctness.

\end{itemize}
	
In order to simplify the code of the algorithm, let us define the following functions:

\begin{itemize}
%\noindent{\bf -} 
\item ${\sf select\_pairs} (echo\_vals_i)$: this function takes as input the set $echo\_vals_i$ and returns tuples $\langle v, sn \rangle$, such that there exist at least $\# echo_{CUM}$ occurrences in $echo\_vals_i$ of such tuple (ignoring the Timer value, if present). 
%\noindent{\bf -} 
\item ${\sf insert}(V_{safe_i}, \langle v_k, sn_k \rangle)$: this function inserts $\langle v_k, sn_k \rangle$ in $V_{safe}$ according with the incremental order and if there are more than $3$ values then the oldest one is discarded. If it is not possible to establish an incremental order, because of ambiguity due to transient failures, then $V_{safe_i}$ is reset.
%: (i) $V_{safe}=\emptyset$ or $\nexists \langle v_j, sn_j \rangle \in V_{safe}:|sn_j-_9sn_k|\geq 3$.\\
%\noindent{\bf -} 
\item ${\sf select\_value}(reply_i)$: this function returns the newest pair $\langle v, sn \rangle$ occurring at least $\#reply_{CUM}$ times in $reply_i$  (ignoring the Timer value, if present).
%\noindent{\bf -}
\item${\sf checkOrderAndTrunc}(V_{safe_i})$: this function checks if it possible to uniquely order the elements in $V_{safe_i}$ with respect to the timestamps, if yes, the $3$ newest element are kept, the others are discharged. If it is not possible to uniquely establish an order for each pair of elements then all the elements are discharged.
%\noindent{\bf -}
\item${\sf checkOrder}(V_{safe_i})$: this function checks if (i) it is possible to establish an unique order for each couple of elements in $V_{safe_i}$. If not, $V_{safe_i}$ is emptied.
%\noindent{\bf -}
\item ${\sf conCut}(V_i, V_{safe_i},W_i)$: this function takes as input three $3$ dimension ordered sets and returns another $3$ dimension ordered set. The returned set is composed by the concatenation of $V_{safe_i} \circ V_i \circ W_i$, without duplicates, truncated after the first $3$ newest values (with respect to the timestamp). e.g., $d=3$, $V_i=\{\ang{v_a}{1},\ang{v_b}{2}, \ang{v_c}{3}\}$ and $V_{safe_i}=\{\ang{v_b}{2}, \ang{v_d}{4}, \ang{v_f}{5}\}$ and $W_i=\emptyset$, then the returned set is $\{\ang{v_c}{3}, \ang{v_d}{4}, \ang{v_f}{5}\}$. If is it not possible to establish and order  in one of those sets because of transient failures then the result in $\bot$.
%\end{itemize}
%\noindent{\bf -} 
\item ${\sf checkTimer}(W_i)$: this function removes from $W_i$ all the values whose associated timer is $0$ or strictly greater than $2\delta$.

\end{itemize}
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % %



\noindent{\bf The ${\sf maintenance}()$ operation.} Such operation is executed by servers periodically at any time $T_i=t_0+i\Delta$. Each server first stores the content of $V_{safe_i}$ in $V_i$ and all $V_{safe_i}$ and $echo\_vals_i$ sets are reset. Each server broadcasts an {\sc echo} message with the content of $V_i$, $W_i$ and the $pending\_read_i$ set. When there is a value in $echo\_vas_i$ set that occurs at least $\#echo_{CUM}$ times, $s_i$ it tries to update $V_{safe_i}$ set by invoking ${\sf insert}$ on the value returned by the ${\sf select\_pairs} (echo\_vals_i)$ function. To conclude, after $\delta$ time since the beginning of the operation, the $V_i$ set is reset. Informally speaking, during the \op{maintenance} operation $V_{safe_i}$ is filled with safe values, then the content in $V_i$ is not more necessary. Notice that the content of $W_i$ is continuously monitored so that expired values are removed.\\

%\begin{figure*}[!]
%\centering
%%	\subfigure[Write Protocol: client side]{
%\fbox{
%\begin{minipage}{0.4\textwidth}
%%\footnotesize
%\scriptsize
%%\renewcommand{\baselinestretch}{2.5}
%\resetline
%\begin{tabbing}
%aaaA\=aA\=aA\=aaaA\kill
%
%${\sf init}()$ :\\
%
%\line{}\> {\bf trigger} ${\sf maintenance}()$; ${\sf checkTimer}(W_i)$; ${\sf select} (echo\_vals_i)$;\\
%
%%\line{} \> {\bf while}(\sc true):\\
%%
%%\line{}\>\> ${\sf select\_pairs} (echo\_vals_i)$;\\
%%
%%\line{}\> {\bf endWhile}\\
%
%%\line{}\> {\bf trigger} ${\sf checkTimer}(W_i)$;\\
%%
%%\line{}\> {\bf trigger}  ${\sf select} (echo\_vals_i)$;\\
%
%%\line{T-01}\> {\bf for each} \= $(\ang{\ang{v}{csn}}{timer}_j \in W_i $) {\bf do}\\
%%
%%\line{T-02} \>\> {\bf if} \= $(Expires(timer) \wedge (timer>2\delta)$\\
%%
%%\line{T-03} \>\>\> $W_i \leftarrow W_i \setminus \ang{\ang{v}{csn}}{timer}_j $;\\
%%
%%\line{T-05} \>\> {\bf endif}\\
%%
%%\line{T-06}\>{\bf endFor}\\
%
%~------------------------------------------------------------------------------------------------------\\
%
%{\bf operation} ${\sf maintenance}()$ {\bf executed every} $T_i=t_0+\Delta_i$ :\\
%
%\line{M-CUM-00} \> ${\sf checkOrderAndTrunc}(V_{safe_i})$;\\
%
%%%\line{M-CUM-01} \> {\bf if} $|W_i| > 4$ \\
%%%
%%%\line{M-CUM-02} \>\> {\bf then} $W_i \leftarrow \emptyset$ \\
%%%
%%%\line{M-CUM-04} \> {\bf endIf};\\
%%%
%%%\line{M-CUM-07} \> {\bf if} $\neg({\sf check}(V_i))$;\\
%%%
%%%\line{M-CUM-08}\>\> {\bf then}$V_i[0] \leftarrow \ang{\bot}{\bot}, V_i[1] \leftarrow \ang{\bot}{\bot}, V_i[2] \leftarrow \ang{\bot}{\bot} $;\\
%%%
%%%\line{M-CUM-09} \> {\bf endif}\\
%
%\line{M-CUM-01} \> $echo\_vals_i\leftarrow \emptyset$; $V_i\leftarrow V_{safe_i}$; $V_{safe} \leftarrow \emptyset$; \\
%
%%\line{M-CUM-02} \> $Set_i \leftarrow \emptyset$;\\
%%
%%\line{M-CUM-03}\> {\bf for each}$ \ang{\ang{v}{csn}}{timer}_j \in W_i$ {\bf do};\\
%%
%%\line{M-CUM-04}\>\> $Set_i \leftarrow Set_i \cup \ang{v}{csn}_j$;\\
%%
%%\line{M-CUM-05}\>{\bf endFor} \\
%
%\line{M-CUM-06} \> ${\sf broadcast}$ {\sc echo}$(i,  V_i \cup W_i, pending\_read_i)$;\\
%%
%\line{M-CUM-06a} \>  {\bf wait}$(\delta)$;\\
%
%\line{M-CUM-06b} \> $V_i \leftarrow \emptyset$;\\
%
%~-------------------------------------------------------------------------------------------------------------\\
%
%{\bf when} \=  {\sc echo} $(j, S, pr)$ \= is  ${\sf received}$: \\ 
%
%%\line{M-CUM-22} \> $echo\_vals_i \leftarrow echo\_vals_i \cup V'$;\\
%\line{M-CUM-12} \> {\bf for each} \= $(\langle v, sn \rangle_j \in S)$\\
%
%\line{M-CUM-13} \>\> $echo\_vals_i \leftarrow echo\_vals_i \cup \langle v, sn \rangle_j$;\\
%
%\line{M-CUM-14} \>  {\bf endFor}\\
%\line{M-CUM-15} \> $echo\_read_i \leftarrow echo\_read_i \cup pr$;\\
%
%~------------------------------------------------------------------------------------------------------\\
%
%{\bf function}  ${\sf select} (echo\_vals_i)$:\\
%
%% % % % % % % % % % % % %
%
%%\line{M-CUM-11} \> {\bf wait}$(\delta)$;\\
%
%%\line{M-CUM-12} \> $V \leftarrow \bot$;\\
%
%\line{} \> {\bf while}(\sc true):\\
%
%\line{M-CUM-13} \>\> {\bf if} \= ${\sf select\_pairs} (echo\_vals_i)\neq \bot$;\\
%
%\line{M-CUM-13} \>\>\> $\ang{v_k}{sn_k} \leftarrow {\sf select\_pairs} (echo\_vals_i)$;\\
%
%%\line{M-CUM-14} \> {\bf while} $set\_tmp \neq \bot$ {\bf do} \\
%
%\line{M-CUM-15}\>\>\> ${\sf insert}(V_{safe_i},  \ang{v_k}{sn_k})$;\\
%
%%\line{M-CUM-16} \>\>$set\_tmp \leftarrow set\_tmp \setminus {\sc older}(set\_tmp)$;\\
%
%%\line{M-CUM-17} \> {\bf endWhile};\\
%
%% % % % % % % % % % % % % % % % % % % % % % % % %
%
%%\line{M-CUM-08}\> ${\sf insert}(V_{safe_i}, {\sf select\_three\_pairs\_max\_sn} (echo\_vals_i) )$;\\
%
%%\line{M-CUM-09} \>{\bf for each} \= $(j \in (pending\_read_i \cup echo\_read_i))$ {\bf do}\\
%
%\line{M-CUM-10} \>\>\> ${\sf send}$ {\sc reply} $(i, {\sf conCut}(V_i,V_{safe_i},W_i)))$ to $c_j$;\\
%
%\line{M-CUM-11} \>\>{\bf endIF}\\
%
%\line{M-CUM-11} \>{\bf endWhile}\\
%%
%
%
%\end{tabbing}
%\normalsize
%\end{minipage}
%}
%\caption{$\mathcal{A}_{M}$ algorithm implementing the ${\sf maintenance}()$ operation (code for server $s_i$) in the $(\Delta S, CUM)$ model with bounded timestamp.}
%\label{fig:stateMaintenanceProtocolCUM}   
%\end{figure*}
%
%%==============================================================================

\noindent{\bf The ${\sf write}()$ operation}. When the \op{write} operation is invoked, the writer increments $csn \leftarrow csn +_m 1$, sends {\sc write}$({v}{csn})$ to all servers and finally returns after $\delta$ time.
For each server $s_i$, two cases may occurs, $s_i$ delivers {\sc write}$(\ang{v}{csn})$ message when it is not affected by a Byzantine agent or when it is affected by a Byzantine agent. In the first case $s_i$ stores $v$ in $W_i$ and forward it to every servers sending the {\sc echo}$(i, \ang{v}{csn}, pending\_read_i)$ message. Such value is further echoed at the beginning of each next \op{maintenance} operation as long as $\ang{v}{csn}$ is in $W_i$ or $V_i$, this is true for $\#echo_{CUM}$ correct servers. When $\ang{v}{csn}$ occurs $\#echo_{CUM}$ times in $echo\_vas_i$ then $s_i$ tries to update $V_{safe_i}$ set by invoking ${\sf insert}$ on the value returned by the ${\sf select\_pairs} (echo\_vals_i)$ function. Since there are $\#echo_{CUM}$ correct servers echoing such value then it is in $V_{safe_i}$ also for servers that where affect when {\sc write}$({v}{csn})$ has been delivered.\\  

\noindent{\bf The ${\sf read}()$ operation}. At client side, when the \op{read} operation is invoked at client $c_i$, it empties the $reply_i$ set and sends to all servers the {\sc read}$(i)$ message. Then $c_i$ waits $2\delta$ time, while the $reply_i$ set is populated with servers replies, and from such set it picks the newest value occurring $\#echo_{CUM}$ times invoking ${\sf select\_value}(reply_i)$ and returns it. Notice that before returning $c_i$ sends to every server the read termination notification, {\sc read\_ack}$(i)$ message. At server side when $s_j$ delivers the {\sc read}$(i)$ message, client $c_i$ identifier is stored in the $pending\_read_j$ set. Such set is part of the content of {\sc echo} message in every \op{maintenance} operation, which populates the $echo\_read_j$ set, so that cured servers can be aware of the reading clients. After, $s_j$ invokes ${\sf conCut}(V_j, V_{safe_i},W_i)$ function to prepare the reply message for $c_i$. The result of such function is sent back to $c_i$ in the {\sc reply} message. Such message is also computed and sent during the \op{maintenance} operation, in order to reply with correct values in the case $s_j$ was affected by Byzantine agent. Finally a {\sc reply} message containing just one value is sent when a new value is added in $W_i$ and there are clients in the $pending\_read_j \cup echo\_read_j$ set. When the {\sc read\_ack}$(i)$ message is delivered from $c_i$ then its identifier is removed from the $pending\_read_j$ and $ echo\_read_j$ sets.




%
%
%
%
%%==============================================================================
%
%\begin{figure*}[!]
%\centering
%%	\subfigure[Client code (code for client $c_i$).]{
%\fbox{
%\begin{minipage}{0.4\textwidth}
%%\footnotesize
%\scriptsize
%%\renewcommand{\baselinestretch}{2.5}
%\resetline
%\begin{tabbing}
%aaaA\=aA\=aA\=aaaA\kill
%
%{\bf operation} ${\sf write}(v)$: ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ \\
%
%%~\\
%
%\line{W-CCUM-01} \> $csn \leftarrow (csn+_m 1)$;\\
%
%\line{W-CCUM-02} \> ${\sf broadcast}$ {\sc write}$(v, csn)$;\\
%
%\line{W-CCUM-03} \> {\bf wait} $(\delta)$;\\
%
%\line{W-CCUM-04} \> {\bf return} ${\sf write\_confirmation}$;
%
%
%
%\end{tabbing}
%\normalsize
%\end{minipage}%
%}
%\label{sfig:writeCCUM}
%% \subfigure[Server code (code for server $s_i$).]{
%\fbox{
%\begin{minipage}{0.4\textwidth}
% 
%% \footnotesize
%\scriptsize
% 
%%\resetline
%\begin{tabbing}
%aaaA\=aA\=aA\=aaA\kill
%
%{\bf when} \=  {\sc write}$(v, csn)$ \= is  ${\sf received}$: \\ 
%
%%\line{W-SCUM-01} \>  ${\sf checkOrder}(\ang{v}{cns}, V_i, V_{safe_i})$;\\
%
%\line{W-SCUM-02} \> $W_i \leftarrow W_i \cup \ang{\ang{v}{csn}}{setTimer(2\delta)}$;\\
%
%\line{W-SCUM-03} \> ${\sf broadcast}$ {\sc echo}$(i, \ang{v}{csn}, pending\_read_i)$;\\
%%non serve perché lo vado a mettere nel set echo che cancello ad ogni inizio di maintenanace, quindi o 
%%lo mando all'inizio o non serve a niente ma serve invece quando \Delta\geq 2\delta.
%
%\line{W-SCUM-04} \>  {\bf for} \= {\bf each} $j \in (pending\_read_i \cup echo\_read_i)$ {\bf do}\\
%
%\line{W-SCUM-05} \> \>  ${\sf send}$ {\sc reply} $(i, \{\langle v, csn \rangle\} )$;\\
%
%\line{W-SCUM-06} \> {\bf endFor}\\
%
%
%\end{tabbing}
%\normalsize
%\end{minipage}
%}
%\label{sfig:writeSCUM}
%
%%\caption{$\mathcal{A}_{Rreg}$ ${\sf write}()$ operation protocol.}
%\caption{$\mathcal{A}_{W}$ algorithms, server side and client side respectively, implementing the ${\sf write}(v)$ operation in the $(\Delta S, CUM)$ model with bounded timestamp.}
%\label{fig:writeProtocolCUM}   
%\end{figure*}
%
%%==============================================================================
%
%
%
%%==============================================================================
%
%\begin{figure}[!]
%\centering
%	%\subfigure[Client code (code for client $c_i$).]{
%\fbox{
%\begin{minipage}{0.4\textwidth}
%%\footnotesize
%\scriptsize
%%\renewcommand{\baselinestretch}{2.5}
%\resetline
%\begin{tabbing}
%aaaA\=aA\=aA\=aaaA\kill
%
%{\bf operation} ${\sf read}()$: ~~ \\
%
%%~\\
%
%\line{R-CCUM-01} \> $reply_i \leftarrow \emptyset$;\\
%
%\line{R-CCUM-02} \> ${\sf broadcast}$ {\sc read}$(i)$;\\
%
%\line{R-CCUM-03} \> {\bf wait }$(T_r)$;\\
%
%\line{R-CCUM-04} \> $\langle v, sn \rangle \leftarrow {\sf select\_value}(reply_i)$;\\
%
%\line{R-CCUM-05} \> ${\sf broadcast}$ {\sc read\_ack}$(i)$;\\
%
%\line{R-CCUM-06} \> {\bf return} $v$;\\
%
%
%~-----------------------------------------------------------------------\\
%
%{\bf when} \=  {\sc reply} $(j, V_{set})$ \= is  ${\sf received}$: \\ 
%
%%\line{R-CCUM-07} \>{\bf if}\=$(|V_{set}|>1)${\bf then}\\
%
%\line{R-CCUM-07} \> {\bf for each}\=  $(\langle v, sn \rangle \in V_{set})$ {\bf do}\\
%
%\line{R-CCUM-08} \>\> $reply_i \leftarrow reply_i \cup \{\langle v, sn \rangle_j \}$;\\
%
%\line{R-CCUM-09} \> {\bf endFor}\\
%
%%\line{R-CCUM-10} \>\>{\bf else} {\bf \% $V_{set}=\langle v, sn \rangle$}\\
%%
%%\line{R-CCUM-11} \>\> $reply_{CW_1} \leftarrow reply_{CW_1} \cup \{\langle v, sn \rangle_j \}$;\\
%%
%%\line{R-CCUM-12} \>{\bf endIf}\\
%
%\end{tabbing}
%\normalsize
%\end{minipage}
%%}
%\label{sfig:readCCUM}
%}
% %\subfigure[Server code (code for server $s_i$).]{
%\fbox{
%
%\begin{minipage}{0.4\textwidth}
% 
%% \footnotesize
%\scriptsize
% 
%%\resetline
%\begin{tabbing}
%aaaA\=aA\=aA\=aaA\kill
%
%{\bf when} \=  {\sc read} $(j)$ \= is  ${\sf received}$: \\ 
%
%\line{R-SCUM-01} \> $pending\_read_i \leftarrow pending\_read_i \cup \{j\}$;\\
%
%\line{R-SCUM-02} \> ${\sf send}$ {\sc reply} $(i, {\sf conCut}(V_i,V_{safe_i},W_i))$;\\
%
%\line{R-SCUM-03} \> ${\sf broadcast}$ {\sc read\_fw}$(j)$;\\
%
%~-----------------------------------------------------------------------\\
%
%{\bf when} \=  {\sc read\_fw} $(j)$ \= is  ${\sf received}$: \\ 
%
%\line{R-SCUM-04} \> $pending\_read_i \leftarrow pending\_read_i \cup \{j\}$;\\
%
%~-----------------------------------------------------------------------\\
%
%{\bf when} \=  {\sc read\_ack} $(j)$ \= is  ${\sf received}$: \\ 
%
%\line{R-SCUM-05}\>$pending\_read_i \leftarrow pending\_read_i \setminus \{j\}$;\\
%
%\line{R-SCUM-06} \>$echo\_read_i \leftarrow echo\_read_i \setminus \{j\}$;
%
%\end{tabbing}
%
%
%
%\normalsize
%\end{minipage}
%%}
%\label{sfig:readSCUM}
%}
%%\caption{$\mathcal{A}_{Rreg}$ ${\sf read}()$ operation protocol.}
%\caption{$\mathcal{A}_{R}$ algorithms, server side and client side respectively, implementing the ${\sf read}()$ operation in the $(\Delta S, CUM)$ model with bounded timestamp.}
%\label{fig:readProtocolCUM}   
%\end{figure}


